Topological Neural Networks: Mitigating the Bottlenecks of Graph Neural Networks via Higher-Order Interactions

The irreducible complexity of natural phenomena has led Graph Neural Networks to be employed as a standard model to perform representation learning tasks on graph-structured data. While their capacity to capture local and global patterns is remarkable, the implications associated with long-range and higher-order dependencies pose considerable challenges to such models. This work starts with a theoretical framework to reveal the impact of network's width, depth, and graph topology on the over-squashing phenomena in message-passing neural networks. Then, the work drifts towards, higher-order interactions and multi-relational inductive biases via Topological Neural Networks. Such models propagate messages through higher-dimensional structures, providing shortcuts or additional routes for information flow. With this construction, the underlying computational graph is no longer coupled with the input graph structure, thus mitigating the aforementioned bottlenecks while accounting also for higher-order interactions. Inspired by Graph Attention Networks, two topological attention networks are proposed: Simplicial and Cell Attention Networks. The rationale behind these architecture is to leverage the extended notion of neighbourhoods provided by the arrangement of groups of nodes within a simplicial or cell complex to design anisotropic aggregations able to measure the importance of the information coming from different regions of the domain. By doing so, they capture dependencies that conventional Graph Neural Networks might miss. Finally, a multi-way communication scheme is introduced with Enhanced Cellular Isomorphism Networks, which augment topological message passing schemes to enable a direct interactions among groups of nodes arranged in ring-like structures.

==> Include/Chapters/2_Background/2.1_topological_concepts.tex <==
\input{Include/Chapters/2_Background/2.1.2_simplicial_compelxes}
\input{Include/Chapters/2_Background/2.1.3_cell_complexes}

==> Include/Chapters/2_Background/deep_learning.tex <==
\section{Deep Learning}



In this chapter we give a general overview on neural networks and their advances, starting from basic definitions and properties, following an overview on neural networks for modelling temporal dependencies in sequences and finally we define the autoencoder model, which is fundamental in the anomaly detection problem.


\subsection{Neural Networks}

A neural network is a mathematical model which works by stacking up layers. In each layer, there are a given number of nodes, which are sometimes called neurons (by analogy with the biological brain). Nodes are simply representations of numbers stored in the program. Starting with the input layer, all the way to the output layer, the values stored (called the activation of the node), say, in the $l^{th}$ layer will be used to compute the values stored in the nodes in the $(l + 1)^{th}$ layer. Mathematically, the activations computed by a layer with $h$ nodes are represented by a vector of dimension $h$. \\

In order to refer to the structure of a specific neural network, the term \textit{depth} is commonly used to refer to the number of hidden layers in the network. Hence, when the terms \textit{deep network} or \textit{deep learning} are used, it mean that a specific network has a large number of layers. Usually we refer to how many nodes there are in each hidden layer of the network with as the \textit{width} of the layer. This term is well defined for networks in which all hidden layers have the same number of nodes, but not so much in networks in which the number of nodes varies from layer to layer. A visual representation of a simple neural network is presented in Fig.~\ref{fig:background:deep_learning:nn}. \\

This system  presents many analogies to biological networks of neurons, in which one neuron firing up (transmitting an electric signal) will fire up (propagate the electric signal) nearby neurons. A significant difference between these two systems is that in biological networks, a neuron is either activated or not, while in artificial neural networks it may have a continuum of activations, such as a real number between 0 and 1 (like in sigmoid networks), a non-negative number (like in ReLU networks), or complex numbers \lgc{Inserire citazione eleonora}. In the beginnings of artificial neural networks, some algorithms attempted to implement a binary activation system, only allowing the values on nodes to be either 0 or 1. However, this approach significantly hindered the efficiency of the learning process. \lgc{Inserire figura biological neuron}


\begin{figure}[t]
\centering
\includegraphics[width=0.9\textwidth]{Figures/Background/Deep_Learning/nn.jpg}
\caption{A visual representation of a neural network shown as a directed weighted graph.\lgc{RIFAI}}\label{fig:background:deep_learning:nn}
\end{figure}

\subsection{Building Blocks: Weights \& Biases}

Given the values stored in the $l^{th}$ layer of the network (with, say, $j$ nodes), the values of the next layer (with, say, $k$ nodes) are computed by giving a specific \textit{connection strength} to each node in the next layer. This \textit{connection strength} is mathematically represented by what is called a weight, which is a real number. For notation, set $w_{j,k}^n \in \mathbb{R}$ as the weight between the $j^{th}$  node in the $(l-1)^{th}$ layer to the $k^{th}$ node in the $l^{th}$ layer. In matrix form:

\begin{equation}
    \mathbf{W}_l = 
    \begin{bmatrix}
    w_{1,1}^l & \cdots & w_{1,k}^l\\
    \vdots & \ddots & \vdots \\
    w_{j,1}^l & \cdots & w_{j,k}^l\\
    \end{bmatrix}
\end{equation}

We may want to consider an additive \textit{bias} term $b \in \mathbb{R}^k$, and an \textit{activation function}, a point-wise non-linear function $\sigma : \mathbb{R} \rightarrow \mathbb{R}$ that maps the outputs of the neurons into a \lgc{CONTINUA}. The activation function is an essential block of the neural network architecture because as stated in the \textit{universal approximation theorem}, a neural networks of the form (eq 2.3 the property to approximate arbitrary real-valued continuous functions defined on compact subsets of $\mathbb{R}^n$. Intuitively, given a general data generating mechanism:

\begin{equation}
    y = f(x) + \varepsilon
\end{equation}

There exist a neural network (shallow or deep it is) which is able to approximate $f(x)$ almost perfectly. The only problem in using a neural network as learning model is that we don't know a priori the architecture able to recover the whole data generating mechanism. . To compute the hidden representation $H_l$ of the $l^{th}$ layer, we have:
\begin{equation}
H_l = \sigma(W_l \cdot H_{l-1}  + b_l) = \sigma 
	\begin{pmatrix}
		\begin{bmatrix}
		    w_{1,1}^l & \cdots & w_{1,k}^l\\
		    \vdots & \ddots & \vdots \\
		    w_{j,1}^l & \cdots & w_{j,k}^l\\
		\end{bmatrix}
		\begin{bmatrix}
		    h_1^{l-1}\\
		    \vdots  \\
		    h_k^{l-1}\\
		\end{bmatrix}
		+
		\begin{bmatrix}
		    b_1^{l}\\
		    \vdots  \\
		    b_j^{l}\\
		\end{bmatrix}
	\end{pmatrix}
\end{equation}

The output of the network, $\hat{f}$ is then computed as the stack of depth $L$ of network's layers:
\begin{equation}
    \hat{f}(\mathbf{x}) = \sigma(W_L \cdot \sigma(\ldots \cdot \sigma(W_2 \cdot \sigma(W_1 \cdot \mathbf{x} + b_1) + b_2) \ldots ) + b_L)
\end{equation}

\subsection{Learning Process}
In a real world scenario, these networks are used to estimate functions which we do not know how to write down analytically (if we did, there would be no need to go though the trouble of setting up a neural network). Although this section does not go in depth regarding the learning process, a rough outline of the most common method of training neural networks will be outlined here. Even though this thesis mostly explores the properties of expressivity of a particular class neural networks, most emphasis and problems regarding the use of these algorithms rely on the training process, and how to obtain the best results given a finite training data set. A neural networks is, after all, a data driven algorithm.

\subsection{Loss Function}
Suppose we want to approximate a function $f : \mathbb{R}^n \rightarrow \mathbb{R}^m$, and our network currently computes a function 
$\hat{f}: \mathbb{R}^n \rightarrow \mathbb{R}^m$. In order to determine how well a certain prediction given by the algorithm is, we may establish a cost function, which measures the discrepancy of two functions. To do that, we can feed some input $x$ of which we know the value of $f(x)$ (this would be called a label data point) to the network and see what result it computes. In a broader sense, we may see how well the network performs on a testing set $(x_1, \ldots,x_N)$ in which we know all the values for $f(x_1), \ldots, f(x_N)$. There is more than one choice for such a function, but for the purpose of this thesis, let's consider the \textit{Mean Squared Error} for \textit{regression} taks:

\begin{equation}
    \mathcal{L} = \frac{1}{N} \sum_{i=1}^N \vert \vert f(x_i) - \hat{f}(x_i))\vert \vert_2^2
\end{equation}




This function, then, becomes large when our network approximates $f$ badly, and small when the approximation is accurate. So, the aim of the learning process is to find out the values $W^*$ and $b^*$ that minimize the cost function. The same holds for \textit{classification} tasks, where  $f: \mathbb{R}^n \rightarrow \{1, \ldots, C\}$ maps each sample into a class. In this case, we use the \textit{Cross Entropy} loss to measure the error that the network $\hat{f}(x_i)$ makes in predicting $y_{i,C}$, the correct sample's class: 


\begin{equation}
    \mathcal{L} = \frac{1}{N} \sum_{i=1}^N  \sum_{c=1}^{C} y_{i,c} - log(\psi(\hat{f}(x_i))),
\end{equation}

where $\psi$ is the softmax function.

\subsection{Gradient Descent}

Gradient descent is a standard method used in optimization problems. It relies on concepts from multivariable calculus.

Given a differentiable scalar function $f : \mathbb{R}^n \rightarrow \mathbb{R}$, the \textit{gradient} of $f$ at a point $x = (x_1, \ldots, x_n) \in \mathbb{R}^n$ is a vector in $\mathbb{R}^n$ of the form:

\begin{equation}
	\nabla f(x) = \left( \frac{\partial f(x)}{\partial x_1}, \ldots, \frac{\partial f(x)}{\partial x_n} \right)
\end{equation}

Given a point $x \in \mathbb{R}^n$, the gradient of $f$ at that point indicates the direction its steepest ascent. Given that $f$ is differentiable at $x$, it can be approximated linearly, and therefore the vector $ - \nabla f(x)$ indicates the direction of steepest descent of the function $f$ at the point $x$. In order to obtain the minimum value of the function, the gradient descent strategy tells us to start at a given $x_0 \in \mathbb{R}^n$, calculate the value of $\nabla f(x_0)$, and then proceed to calculate a new point $x_1 = x_0 - \alpha \nabla f(x_0)$, where $\alpha > 0 $ is called the learning rate. We then repeat this process, creating a sequence $\{x_i\}$ defined by our initial choice of $x_0$, the learning rate $\alpha$, and the rule: $x_{i+1} = x_i - \alpha \nabla f(x_i)$ for any $i \in N$. This sequence continues until we approach a region of the loss landscape close to our desired minimum. \lgc{Insert stochastic gradient descent and batch gradient descent} - \lgc{Insert that modern optimization process i.e., adam are just refinements of SGD}. Let us define the loss function as the sum over the losses computed for a single sample:

\begin{equation}
\mathcal{L} = \sum_{i=1}^N \mathcal{L}_{x_i}
\end{equation}


By the linearity property of the derivative we have that:

\begin{equation}
    \nabla \mathcal{L} = \nabla \left( \sum_{i=1}^N \mathcal{L}_{x_i} \right) = \sum_{i=1}^N \nabla \mathcal{L}_{x_i}
\end{equation}

which means that we can execute this process for each data point and then add the values of the gradient together. This is important because employing backpropagation in a large training set for every training epoch becomes a very computationally expensive approach. Instead we select one (for \textit{Stochastic Gradient Descent}) or a batch of elements (hence \textit{Batch Gradient Descent} from the training set, compute the gradients, update the network's weights and biases and repeat the process until it arrives at satisfactory results.





\subsubsection{Backpropagation}

In this section we will give a brief explaination to the method of \textit{backpropagation} in neural networks which, without loss of generality, is an algorithm used to compute the gradients of the cost function with respect to the neural networks trainable parameters. The proof of some equations will only be sketched, as they are not related to the mathematics of the expressive power of networks, which forms the bulk of this work. For a more comprehensive understanding of the backpropagation algorithm, we refer the reader to~\cite{goodfellow2016deep}. The challenge of applying gradient descent to neural networks is calculating the partial derivatives of the cost function with respect to each individual weight and bias (namely, for every $\partial w_{i,j}^l$ and $\partial b_j^l$. This is where the backpropagation comes in. This algorithm first tells us how to calculate these values for the last layer of connections, and with these results then inductively goes \textit{backwards} through the network, calculating the partial derivatives of each layer until it reaches the first layer of the network. 


In a previous section, we defined $a_n$ to be the vector representing the activations of the nodes in the $n^{th}$ layer of the network. However, for the purposes of this section, it will be useful for us to consider what the values sent by the previous layer were before the activation function was applied. Consider

\begin{equation}
    z_j^l = \sum_k w_{j,k}^l h_k^{l-1}+ b_l^l \qquad \text{s.t.}  \qquad
    h_j^l = \phi(z_j^l) 
    \qquad and \qquad
    H^l = \sigma(Z^l) \notag
\end{equation}

In the previous equation, $Z_l = \sum_k z_k^l e_k$ is a vector with entries corresponding to the values $z_j^l$ ($e_k$ are the standard basis vectors). Additionally, consider the quantities

\begin{equation}
    \delta_j^l = \frac{\partial L}{\partial z_j^l} 
    \qquad and \qquad
    \Delta^l = \sum_k \delta_k^l e_k \notag
\end{equation}

These values will be useful for propagating the algorithm backwards through the network and are directly related to $\frac{\partial \mathcal{L}}{\partial w_{i,j}^l}$ and $\frac{\partial \mathcal{L}}{\partial b_j^l}$ using the chain rule, since:

\begin{equation}
    \frac{\partial \mathcal{L}}{\partial w_{i,j}^l} = 
    \frac{\partial \mathcal{L}}{\partial z_j^l} \frac{\partial z_j^l}{\partial w_{i,j}^l} = 
    \delta_j^l a_i^{l-1} 
    \qquad and \qquad
    \frac{\partial \mathcal{L}}{\partial b_j^l} = 
    \frac{\partial \mathcal{L}}{\partial z_j^l} \frac{\partial z_j^l}{\partial b_j^l} = 
    \delta_j^l \notag
\end{equation}

Since $ a_j^{l-1}$ is readily available for any node of the network, if we are able to calculate the value of the $\delta_j^l$’s we will have been successful in obtaining our gradient! Our first step is calculating this value for the last layer of the network, that is, $\delta_j^L$ for a network with $L$ layers. It is not hard to notice that, since $a_j^L = \phi(z_j^L)$,
again by the chain rule:

\begin{equation}
    \delta_j^L = \frac{\partial C}{\partial a_j^L} \frac{\partial a_j^L}{\partial z_j^L} = 
    \frac{\partial C}{\partial a_j^L} \phi^{'}(z_j^L)
    \notag
\end{equation}

Using the Mean Square Error as cost function, noticing that $F(X) = A^L = (a_1^L, \ldots, a_k^L)$ and letting $f(x) = (y_1, \ldots, y_k)$ we get that:

\begin{equation}
    \delta_j^L = (a_j^L-y_j) \phi^{'}(z_j^L)
    \notag
\end{equation}

So, if we are able to compute $\phi^{'}(\cdot)$, the value $\delta_j^L$ can be easily computed too. In order to vectorize the computation, it is common to write:

\begin{equation}
    \Delta^L = \nabla_{A^L} \odot \phi^{'}(Z^L)
\end{equation}\label{deltas}

where $\nabla_{A^L} = (\frac{\partial C}{\partial a_1^L}, \ldots, \frac{\partial C}{\partial a_k^L})$ is the gradient of the cost function take with respect to all the elements of $A^L$ and $\odot$ is the \textit{Hadamard Product}.
Now we will only need to "propagate" this backwards in the network in order to obtain $\delta_j^{L-1}$. In order to do so, apply the chain rule once again:

\begin{align}
    \delta_j^{L-1} &= \frac{\partial C}{\partial z_j^{L-1}} \\
    &= \nabla{Z^L} C \cdot \frac{\partial Z^L}{\partial z_j^{L-1}} \\
    &= \sum_{i=1}^k  \frac{\partial C}{\partial z_j^L} \frac{\partial z_i^L}{\partial z_j^{L-1}} \\
    &= \sum_{i=1}^k \delta_i^L \frac{\partial z_i^L}{\partial z_j^{L-1}}
\end{align}

Expanding the term $\frac{\partial z_i^L}{\partial z_j^{L-1}}$ we find out that:

\begin{align}
    \frac{\partial z_i^L}{\partial z_j^{L-1}} 
    &= \frac{\partial \left( \sum_k w_{i,k}^L a_k^{L-1} + b_i^L \right) }{\partial z_j^{L-1}} \\
    &= \frac{\partial \left( \sum_k w_{i,k}^L \phi(z_k^{L-1}) + b_i^L \right)}{\partial z_j^{L-1}} \\
    &= \frac{\partial w_{i,j}^L \phi(z_j^{L-1}) }{\partial z_j^{L-1}} \\
    &= w_{i,j}^L \phi^{'}(z_j^{L-1})
\end{align}

Which finally leads to:

\begin{equation}
     \delta_j^{L-1} = \sum_{i=1}^k \delta_i^L w_{i.j}^L \phi^{'}(z_j^{L-1})
\end{equation}

The above equation tells us how to compute any $\delta_j^l$ in the network, assume we know the values $\Delta^{l+1}$. Since \ref{deltas} tells us how to jump start $\Delta^L$ in the last layer of the network, we simply have to compute the first value and then propagate it trough the network by the application of the chain rule.


As shown in~\cite{wolpert1997no}, the \textit{no free lunch theorems} state that any learning algorithm that searches for an optimal loss is not universally superior to any other algorithm. This is due to the huge potential problem space for the application of the general-purpose algorithm; if an algorithm is particularly adept at solving one class of problem, and the fitness surface that comes with it, then then it has to perform worse on the remaining average of problems: \textit{“If an algorithm performs better than random search on some class of problems then in must perform worse than random search on the remaining problems.”}. Because of the no free lunch theorems proof, we can state that a superior black-box optimisation strategy is impossible. So, the choice of using a neural network instead of any other learning model is due to their expressivity power, which can be summarized with the following statement: \textit{The complexity of the computable function grows exponentially with network depth}. 

==> Include/Chapters/2_Background/deprecated_related_works.tex <==
\section{Related Works}\label{sec:rel_works}


In \cite{ebli2020simplicial}, the authors introduce a novel type of neural network architecture, called simplicial neural networks (SNNs), that can process data living on simplicial complexes - a generalization of graphs that can encode higher-order interactions between vertices, allowing for richer data representation and analysis. The authors define an appropriate notion of convolution and leverage it to construct SNNs, which they test on imputing missing data on coauthorship complexes, achieving competitive results compared to state-of-the-art methods. 

In \cite{yang2021simplicial}, they propose a simplicial convolutional neural network (SCNN) architecture for learning from data defined on simplices, and studies its permutation and orientation equivariance, complexity, and spectral analysis, and tests its performance for imputing citations on a coauthorship complex.

In \cite{bodnar2021weisfeiler}, they propose Message Passing Simplicial Networks (MPSNs), a class of models that perform message passing on simplicial complexes to capture multi-level interactions in complex systems, and introduces a Simplicial Weisfeiler-Lehman (SWL) colouring procedure to distinguish non-isomorphic simplicial complexes and analyze the expressivity of the model, which is shown to be strictly more powerful than the WL test and not less powerful than the 3-WL test, and compares MPSNs with traditional graph neural networks in terms of their representational power.

In \cite{bodnar2021weisfeilercell} they decouple the computational graph from the input graph structure through message passing on regular Cell Complexes, resulting in a set of graph "lifting" transformations that lead to a unique hierarchical message passing procedure called CW Networks (CWNs), which are shown to be strictly more powerful than the WL test and not less powerful than the 3-WL test.

In \cite{hajij2020cell} they propose Cell Complex Neural Networks (CXNs), a general, combinatorial, and unifying construction for performing neural network-type computations on cell complexes, and introduces an inter-cellular message passing scheme on cell complexes that takes the topology of the underlying space into account and generalizes message passing scheme to graphs.




==> Include/Chapters/3_Bottlenecks/3.2_Learn_to_Rewire.tex <==
\section{Context Aware Differentiable Rewiring}\label{sec:learn2rew}

A problem affects all standard MPNNs, effectively preventing them from reliably sending messages across nodes at high diffusion distance \citep{xu2018representation, alon2020bottleneck, topping2022understanding}. There's a desire to develop a framework that leverages the information provided by the input graph $\gph$ in terms of differentiating between local vs non-local, all while addressing the over-squashing issue. Consequently, one cannot fix over-squashing within the $\MPNN$ class merely by stacking numerous layers. As $m$ increases, from the minute sensitivity of a node to distant features, there emerges a reduced sensitivity of the entire network. Expanding on \Cref{cor:bound_MLP_MPNN}, it's demonstrated that $\MPNN$ find it challenging to exchange information among nodes with high effective resistance. This realization leads to two vital outcomes: (i) $\MPNN$ showcases a strong inductive bias in favor of prioritizing information from nodes at low effective resistance. (ii) The spectral methods described in \Cref{sec:preliminaries_mpnns} prove successful in countering over-squashing. The discussion begins with a review of essential graph theory concepts. The proposal emphasizes on "scale separation", a tactic best described as 'prioritizing first over local messages, followed by non-local messages without mixing resolutions'. Typically, local MPNNs are frameworks wherein the node update $\mathbf{h}_{v}^{(t)}$ at layer $l$ depends solely on $\mathcal{N}(v)\cup{v}$. 

\

An $\MPNN$ incorporates two main components: the neural network architecture and the graph topology. The investigation focuses on the impact of both components in either mitigating or accelerating the over-squashing phenomenon. This includes an examination of the $\MPNN$'s width, depth, and the graph topology, employing both spatial and spectral techniques to either alleviate or expedite over-squashing. A new GNN framework is introduced, enhancing any $\MPNN$ model to facilitate interactions among node features that might otherwise be overshadowed in the architecture, regardless of layer count. The class of $\tel$ is then introduced, presenting a solution less prone to over-squashing, more potent than $\MPNN$, and as efficient as any chosen $\MPNN$ variant. This approach offers a notable speed advantage over other frameworks crafted to manage long-range interactions or introduce robust GNN structures. Key objectives include: (i) Addressing over-squashing to manage information potentially overlooked by the $\MPNN$. (ii) Counteracting the vanishing/exploding gradient phenomenon. (iii) Prioritizing efficiency and scalability with a training approach that mirrors the chosen $\MPNN$ architecture's timeframe per epoch, without significant spatial-complexity overhead. It's worth noting the increased relevance of this issue of long-range interactions and scalability, especially with the growing interest in graph-transformers.




%%%%%%%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%%%%%%%%


Characterization of hybrid variant 

\paragraph{Context aware learnable rewiring} This strategy represents a multi-resolution approach to generalize $\MPNN$ where information that has been exploited at fine (local) scales by a message-passing architecture, is then sent across coarser scales using the computational templates $\mathcal{R}(\Anorm^{k})$. This partly resonates with existing works that aim at changing the computational graph (i.e. the message-passing template) rather than the architecture. Differently from~\citet{topping2022understanding}, the rewiring here occurs {\em after} (and not {\em before}) the $\MPNN$ hence allowing the latter to learn any (local) structural representation from the input topology. While this approach is in spirit similar to \citet{alon2020bottleneck, deac2022expander, arnaiz2022diffwire}, the key difference is that through the powers $k$ entering the polynomial $\poly$, {\em is possible to access and alter different resolutions of the graph without necessarily modifying the local aggregation computed by} $\MPNN$.


%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%
\subsection{An efficient remedy to over-squashing: the $\ourname$ framework}\label{sec:poly}
In~\Cref{sec:on_oversq} it is provided a unified framework for showing that both spatial and spectral methods discussed in~\Cref{sec:related_work} do alleviate over-squashing. Here it is proposed a novel framework, show that it mitigates over-squashing while adding minimal computational overhead, and comment on the differences with existing approaches. %We assume that we are given a task with long-range interactions that we know $\MPNN$ might be failing to capture due to over-squashing. 
In particular, {\em any} $\MPNN$ can be enhanced by also propagating information on a rewired graph $\rew(\gph)$ that is built by connecting nodes that struggle to exchange information due to over-squashing as per our analysis. %have (approximately) high Jacobian distance as per \Cref{sec:theory_2}. %Such enhancement is achieved with very little overhead that can be absorbed as pre-computation. %, in light of our theoretical analysis, we know to be st whose representations will roughly be independent inside the $\MPNN$ architecture. 
%Put it differently, working on the assumptions that any $\MPNN$ manages to exchange information among nodes `close' to each other, we help any model by allowing it to see those nodes whose messages would otherwise be squashed.
To start, % motivate the introduction of a new class, we start from a simplified case. 
assume a GCN model~\citep{kipf2017graph} with $m$ layers. By removing the nonlinearity, the final representations can be written as a polynomial $\Hi^{(m)} = \sum_{k = 0}^{m}\Anorm^{k}\Xnorm\mathbf{W}^{(k)}$, 
% \begin{equation}\label{eq:poly-GCN}\vspace{-1mm}
%     \Hi^{(m)} = \sum_{k = 0}^{m}\Anorm^{k}\Hi^{(0)}\mathbf{W}^{(k)},
% \end{equation}
\noindent for a set of {\em learnable} weight matrices $\{ \W^{(k)}\} : \W^{(k)} \in \R^{d \times d}$. A natural approach to capture long-range interactions would be to take the degree $m$ large enough. % and, ideally, learn matrices $\mathbf{Q}^{(k)}$ that weight the higher powers $\Anorm^k$ more. 
However,~\Cref{cor:bound_MLP_MPNN} shows how over-squashing occurs precisely due to entries of $\Anorm^k$ decaying exponentially with $k$ for nodes that are far away and badly connected.
Namely, consider two nodes $v,u$ at distance $r$. The interaction between $v$ and $u$ only occurs for powers $\Anorm^{k}$ with $k\geq r$, and is weighted by a quantity approximated by (for $k \sim r$)
\begin{equation}\label{eq:approximation_oversquashing}
(\Anorm^{k})_{vu} \sim \frac{| \{ \pi: v\rightarrow u, \,\, \mathrm{len}(\pi) = k\}|}{d_{\mathrm{avg}}^{r}},
\end{equation}
\noindent where $\pi:v\rightarrow u$ is any path from $v$ to $u$. Accordingly, nodes that are distant from each other, with only few long paths connecting them, are essentially failing to properly exchange information since the denominator grows exponentially with the distance $r$, which describes, in a nutshell,  %which captures 
the over-squashing phenomenon studied in the previous section and in \citet{alon2020bottleneck,topping2022understanding}.
{\em Therefore, %even if the range $k$ is large enough, 
using the same message-passing template $\Anorm$ to propagate information through powers, is bound to lead to over-squashing}. % arising with the powers $\Anorm^{k}$. 
%Since we have identified the cause of over-squashing in Eq.~\eqref{eq:poly-GCN}, 


\


This section proposes a solution to {\em correct} the diffusion operators $\Anorm^{k}$ with alternative ones. % so to allow `badly connected'' pairs of nodes $v,u$ to be coupled by a quantity that is not scaling as Eq.~\eqref{eq:approximation_oversquashing}. 
%We first introduce a way of {\em correcting} the diffusion operators $\Anorm^{k}$. 
\begin{definition}\label{def:poly}
%Consider a graph $\gph$. 
Let $\mathcal{R}:\R^{n\times n} \rightarrow \R^{n\times n}$ be a rewiring map. Given features $\Hi\in\R^{n\times d}$ and weights $\{\W_k\} :  \W_k \in \mathbb{R}^{d\times d}$, the {\em rewired diffusion} induced by %re-weighting map 
$\mathcal{R}$ is 
\begin{align}\label{eq:corrected_poly}
\mathsf{p}\left(\mathbf{H}\right) &=  \sum_{k = 0}^{K}\mathcal{R}(\Anorm^k)\mathbf{H}\W_k
%\sum_{k = k_0}^{k_1-1} \Anorm^{k}\mathbf{H}\W_k + \sum_{k = k_1}^{K}\mathcal{R}(\Anorm^k)\mathbf{H}\W_k.
\end{align}
%\noindent with $\Hi\in\R^{n\times f}$ the features and $\{\W_k\}\subset\R^{f\times f}$ learnable. % channel-mixing matrices. % we usually omit writing the explicit dependence on $\{\W_k\}$ in $\poly$.
\end{definition}
\noindent To avoid cumbersome notations, the dependence of $\poly$ on $\mathcal{R}$ and $K$ is omitted. In this setting, nodes $v,u$ interact according to $\mathcal{R}(\Anorm^k)_{vu}$ for $k$ large enough.
% suitable choices of $\mathcal{R}$ lead to better coupling among nodes whose messages would otherwise be squashed. 
To motivate the choice of $\mathcal{R}$, consider a node $v$. According to \Cref{cor:bound_MLP_MPNN}, the values $\{(\Anorm^k)_{vu}\}_{u\in\V}$ roughly control the exchange of information between $v$ and $u$ in an $\MPNN$ after $k$ layers. If a node $u_{0}$ is `badly connected' to $v$ as per~\Cref{cor:over-squasing_distance}, then the entries $(\Anorm^k)_{vu_0}$ are exponentially small. On the other hand, if $v$ and $u_1$ are at low effective resistance, then there generally are many walks between these two nodes, meaning that $(\Anorm^k)_{vu_1}$ will be much larger than $(\Anorm^k)_{vu_0}$. Since the connectivity provided by $\Anorm^k$ must be altered so that nodes at high-effective resistance can communicate {\em when} the power $k$ is large enough,  $\mathcal{R}$ is chosen to act elementwise as $(\mathcal{R}(\Anorm^k))_{vu} =  \tilde{\mathcal{R}}((\Anorm^k)_{vu})$ if $(\Anorm^k)_{vu} > 0 $, 
two nodes $v,u$ at distance $r$. For $k \sim r$, $(\Anorm^k)_{vu}$ is, approximately, the probability of a random-walk starting at $v$ to arrive at $u$ in $k$ steps. 
\paragraph{The choice of $\mathcal{R}$.} To explain the role of $\mathcal{R}$, take nodes $v,u,\tilde{u}$ at distance $d_{\gph}(v,u) = r >> d_{\gph}(v,\tilde{u})$. The entry $(\Anorm^{k})_{vu}$ is generally much smaller, for $k \sim r$, than $(\Anorm)^{k}_{v\tilde{u}}$, since there are many more paths of length $\mathcal{O}(r)$ from $v$ to $\tilde{u}$ due to {\em random-walk backtracking and being trapped in high-density regions}. Accordingly, $\{\mathcal{R}(\Anorm^{k})\}$ should change only the aggregation for $k$ larger than some local range of interactions $k_0$ by re-weighting the contributions for nodes whose coupling $(\Anorm^k)_{vu}$ is too small, and viceversa. % right hand side of \Cref{eq:approximation_oversquashing} is large and viceversa when the latter is small. 
Let's consider a class of functions of the form
\begin{equation}\label{eq:pointwise-correction}
    (\mathcal{R}(\Anorm^k))_{vu} = \begin{cases} &\nu_{v}\tilde{\mathcal{R}}((\Anorm^k)_{vu}), \,\, \text{if} \,\, (\Anorm^k)_{vu} > 0 \\ 
    &0, \,\, \text{otherwise}
    \end{cases}
\end{equation}
for $\tilde{\mathcal{R}}:\R_{+} \rightarrow \R_{+}$ {\em monotonically decreasing}: in this way, % This choice allows us to inject a strong inductive bias in our framework, since 
the corrected diffusion operators emphasize precisely thee interactions that would be mostly ignored due to over-squashing. Further, since the correction is elementwise, the polynomial $\poly$ is {\em equivariant}. 
In this section, a family $\{ \tilde{\mathcal{R}}^{\theta}_{k}\}$ depending on learnable parameters $\theta$ are considered. However, it is possible to restrict the specific choices of $\tilde{\mathcal{R}}$ to grant a significant computational advantage. %, unless otherwise stated, we restrict to the specific choice of $\mathcal{R}$ in \Cref{eq:LSE}
and reserve generalizations to future work. 
, so that a suitable rewiring map $\mathcal{R}$, can avoid the over-squashing effect in~\Cref{eq:approximation_oversquashing} and the choice of $\mathcal{R}$ is discussed below. 
Let's now introduce the new class of $\tel$ that is built as a framework extending any instances of $\MPNN$ to compensate over-squashing phenomena.

\begin{definition}\label{def:tele} Given %an attributed graph $\mathsf{G}$ and 
an $\MPNN$, compute the embedding $\mathbf{H}_{\mathrm{loc}}^{(m)} = \MPNN^{(m)}(\gph,\mathbf{H}^{(0)})$ after $m$ layers. Given a map $\com$, set $ \tel(\gph,\Hi^{(0)}) := \com(\mathbf{H}_{\mathrm{loc}}^{(m)},\poly(\mathbf{H}^{(0)}))$.
% \begin{equation*}
%     \tel(\gph,\Hi^{(0)}) := \com(\mathbf{H}_{\mathrm{loc}}^{(m)},\poly(\mathbf{H}^{(0)})).
% \end{equation*}   
\end{definition}
\noindent Usually, $\com$ is taken to be a convex combination 
% so that 
% \[ 
% \tel = \alpha \MPNN^{(m)} + (1-\alpha)\poly,
% \]
\noindent and a non-linear readout is applied at the end. Therefore $\tel$ combines, in a {\em decoupled} fashion, {\em any} $\MPNN$, which by \Cref{thm:effective_resistance} has most likely been able to capture relations among low effective resistance nodes, {\em and} a polynomial on corrected diffusion operators that aims at exchanging information precisely among nodes whose information would otherwise be over-squashed as per \Cref{cor:over-squasing_distance}. % at high effective resistance whose messages would be squashed in the $\MPNN$. We stress how this approach extends any existing instances of $\MPNN$. 
%We now validate theoretically that $\tel$ along with the choice of correction described above, can alleviate over-squashing. %Take a pair of nodes $v,u$ at distance $r$. 
% We show that %, if we consider an $\MPNN$ suffering from over-squashing due to the Jacobian decaying exponentially with the distance $r$ as in \Cref{cor:over-squasing_distance}, 
% the corrected polynomial in \Cref{def:poly} has sensitivity bounded from below independent of the distance. %tcan still exchange messages more reliably. 
% Below $\mathcal{R}$ is a decreasing function acting elementwise on $\Anorm^k$. %onsider corrected polynomials as in Eq.~\eqref{eq:pointwise-correction}, where $\tilde{\mathcal{R}}:\R_{+}\rightarrow \R_{+}$ is monotonically decreasing.

% \begin{proposition}\label{prop:tel-over-squashing}
% Let $v,u$ s.t. $d_{\gph}(v,u) = r$ . Assume that $(\Anorm^{r})_{vu} < \delta^{r}$, for $\delta \in (0,1)$. % such that $c_{\up}\omega^{\infty}_{r}c_{\mpas}\delta := \mu < 1$. 
% Let $\tilde{\Hi} = \poly(\mathbf{H}^{(0)})$. There exist $\{\mathbf{W}^{(k)}\}$, with $\max_{k}\lvert\lvert\mathbf{W}^{(k)}\rvert\rvert_{\mathrm{max}} \leq q$ and $\mu > 0$, independent of $r$, such that %for any $\alpha,\beta \in [f]$ we have 
% $\lvert\lvert \partial\tilde{\mathbf{h}}_{v}/\partial \mathbf{h}_{u}^{(0)}\rvert\rvert_{L_1}  > fq\mu$.
% % \begin{equation*}
% %     \left\vert \frac{\partial (\mathsf{p}^{\mathcal{R}, r}_{k_0,k_1}(\mathbf{H}^{(0)}))_{v}^{\alpha}}{\partial \mathbf{h}_{u}^{(0),\beta}}\right\vert  > q\mu.
% % \end{equation*}
% \end{proposition}
\noindent One advantage of the $\tel$-framework then consists in allowing distant and `badly-connected' nodes, intended as those such that the right hand side of Eq.~\eqref{eq:upper_bound_mlp} is decaying exponentially with $m$, to propagate information among them.

% \todo{This paragraph is still to be written: depends on expressivity, time and space} \paragraph{Expressive power: beyond distance information} \textcolor{blue}{Here we can mention the difference with SPN and that this framework in principle sees information beyond the distance. We observe that the choice $\sigma = \pi_{1}$ in \Cref{def:tele} highlights that $\MPNN$ is a subset of $\tel$. In fact, $\tel >$ 1-WL, meaning that the inclusion $\MPNN \subset \tel$ is {\em strict}. It might be worth inserting here an example of regular graphs that can be distinguished by the $\tel$ to shed light on the role of $\mathcal{R}$ and how this may already be no longer described in the $\MPNN$ class. Difference between topological representations?}

{\bf On the complexity of $\tel$.} To account for long-range interactions, intended as those among high effective-resistance nodes as per \Cref{thm:effective_resistance}, some computational price is necessary. Our `enhancement' framework though, has only a marginal overhead. Similarly to \citet{frasca2020sign}, $\mathcal{R}(\Anorm^{k})\mathbf{H}^{(0)}$, can be {\em pre-computed} and stored for lated use so that the complexity of %the forward pass of 
$\poly$ scales with {\em nodes} rather than {\em edges}, becoming $\mathcal{O}(Knf^{2})$. This means that the forward-time is dominated by that of the chosen $\MPNN$ running in parallel. The computational overhead in the pre-processing depends on the density of the matrices $\mathcal{R}(\Anorm^{k})$. Also notice that this is all done {\em outside} the training pipeline. 

\

{\bf An interpretation from the graph-rewiring perspective.} %According to the discussion of related work in \Cref{sec:preliminaries}, here too we take on the point of view of graph-rewiring to comment on the novelty of our approach. 
Differently from pre-processing methods such as \citet{klicpera2019diffusion,topping2022understanding,arnaiz2022diffwire,karhadkar2022fosr}, $\tel$ aggregates information over {\em both} the input graph $\gph$ and a rewired one $\rew(\gph)$. In fact, $\mathcal{R}(\Anorm^k)$ can be identified with different {\em message-passing templates} that only change the computational graph at a certain range, rather than at each layer, as instead done in \citet{bruel2022rewiring, abboud2022shortest}. This partial decoupling allows the framework to leverage the $\MPNN$ to capture local interactions, while also exchanging information {\em precisely} among those nodes whose communication would be over-squashed. While this is similar to \citet{deac2022expander}, where the aggregation is independently computed over $\gph$ and an ideal expander $\gph_{\mathrm{exp}}$, two key differences exists: (i) $\gph_{\mathrm{exp}}$ is constructed independent of the input graph, meaning that the connectivity among {\em any} pairs of nodes is improved, something that can add redundancy, and leaves some ambiguity in the labelling of the nodes of $\gph_{\mathrm{exp}}$. On the other hand, in $\tel$ a node $v$ is enhanced with the ability to 'see' precisely those nodes that would be failed to be captured by the $\MPNN$. (ii) Given two graphs $\gph_1,\gph_2$, the expander construction is the same. In our case instead, the variation of the corrected polynomials in the two cases can be quantified based on the choice of $\mathcal{R}$ and the distribution of the diffusion operators $\{\Anorm^k_1\}$ and $\{\Anorm^k_2\}$. This means that {\em graphs whose diffusion operators are similar, will receive similar corrections, and viceversa}.  




==> Include/Chapters/3_Bottlenecks/On_Graph_Transformer_Networks.tex <==
\section{On Graph Transformer Networks}\label{sec:bottlenecks:on_graph_transformers}

==> Include/Chapters/5_Experiments/5.1.2_exp_learn2rewire.tex <==
\section{Experiments Learn to Rewire}

In this section, we first evaluate the performance of the proposed architecture and training procedure on the authorship attribution learning task, as described in \cite{Segarra_2015}; then, we apply the proposed strategy to a source localization problem on a real-world graph composed of 234 Facebook users~\citep{faceookego}. The proposed method is compared with the following state of the art architectures, namely, (i) Selection GCN, (ii) Aggregation GCN  (iii) Multinode GCN~\citep{gama2018convolutional}, and (iv) Graph coarsening based GCN~\citep{defferrard2016convolutional}. In all the simulations, we used an AA-GCN made of two layers~(\Cref{Auto_GCNN_layer}) with ReLU non-linearities, encoding functions $f_l^e$ with one hidden layer, and a final fully-connected layer with Softmax for classification purposes. We trained our model using Algorithm 1, and exploiting the ADAM optimizer~\citep{kingma2014adam}. Training is performed as in \Cref{GCN_prob_A} for AA-GCNs, and as in \Cref{GCN_classic_prob} for the competitors, where $\mathcal{L}$ is the $\ell_2$ regularized cross-entropy; all the hyper-parameters are tuned via cross-validation. 

\subsection{Benchmarks and Datasets}

\paragraph{Authorship Attribution} For the setup of this simulation, we have followed the settings of \cite{gama2018convolutional}. In particular, the learning task consists in deciding if an extract of a contemporary author's work from the $19^{\textrm{th}}$ century is written by him/her or not. We focus on texts authored by Emily Bront\"{e}. We consider a corpus of $682$ excerpts of $1000$ words, written by her, taking into account $N=211$ functional words, composing a word adjacency network (WAN) graph. We construct a training and a test set made of excerpts belonging to Bront\"{e} and other authors. Each sample can be interpreted as a signal defined over the WAN graph, where the value associated to each node is the frequency count of that specific functional word.



\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.40\textwidth}
         \centering
         \centerline{\includegraphics[width=.99\linewidth]{Figures/Experiments/Acc_N.pdf}}
         \caption{Accuracy vs compression ratio ($\rho$), authorship attribution. }\medskip
         \label{fig:rho_vs_acc}
     \end{subfigure}
     \hspace{.5cm}
     \begin{subfigure}[b]{0.40\textwidth}
         \centering
         \centerline{\includegraphics[width=.99\linewidth]{Figures/Experiments/acc_sigma.pdf}}
         \caption{Accuracy vs $\textrm{SNR}$, source localization on Facebook graph.}\medskip
         \label{fig:rho_vs_sigma}
     \end{subfigure}
     
    \caption{Results on learnable connectivity}
    \label{fig:aa-gcn-results}
\end{figure}


\paragraph{Source Localization} For the source localization task, the goal is to detect the community of source nodes that diffuse information over the network.
We  consider a real-world graph composed of 234 Facebook users~\citep{faceookego}. In particular, we denote by $\boldsymbol{\delta}_c$ the graph signal that contains a 1 value in the position associated to a node belonging to community $c$, and 0 at every other node. Then, let $\mathbf{x} = \mathbf{A}^t \boldsymbol{\delta}_c$ be the diffused graph signal, for some unknown $t \geq 0$. Thus, given $\mathbf{x}$, the goal is to estimate the community $c$ that originated the diffusion. This is clearly a classification problem in which we observe a graph signal $\mathbf{x}$ and have to assign it to one of the 5 communities. 

\subsection{Comparative Performance Analysis}

\input{Tables/acc_learn_to_rewire_authorship}

\paragraph{Authorship Attribution} 

For this experiment, we set $F_1=F_2=32$, $K_1=K_2=5$ and $N_1 = N_2 = 100$. The simulations are averaged over $10$ independent dataset realizations. As a first result, in~\Cref{tab:authorship} we compare the accuracy of the proposed method against the aforementioned competitors. The proposed method obtains a $2\%$ improvement with respect to the best competitor, i.e., Graph coarsening from \cite{defferrard2016convolutional}. Moreover, in Fig. 2, we illustrate the trade-off between compression and accuracy of the proposed architecture, showing the classification accuracy versus the compression factor $\rho := \frac{N_1}{N}$. The proposed AA-GCN is compared with the selection GCNs (Degree and EDS)~\citep{gama2018convolutional} and the graph coarsening architecture~\citep{defferrard2016convolutional} (taken as benchmark, due to its possibility of compressing only at $N_l = N_{l-1}/2$). From Fig. 2, we notice that the proposed architecture leads to the best performance, showing excellent robustness to compression (i.e., enhancing its scalability).

\paragraph{Source Localization}

The hyperparamters of all the compared GCN architectures are: $F_1=F_2=32$,  $K_1=K_2=5$, and $N_1=N_2=10$. We trained the networks for $40$ epochs with batches of $100$ noisy training samples. Since the data realizations are random, we generate $10$ different dataset realizations, and the results are averaged accross the data realizations and graph realizations. In particular, training signals are generated as  $\mathbf{x} = \mathbf{A}^t \boldsymbol{\delta}_c + \boldsymbol{\epsilon}$, where $\boldsymbol{\epsilon}$ is white Gaussian noise with variance $\sigma^2_{\epsilon}$, whose components are independent from the others and from the signal. In Fig. 3, we illustrate the best classification accuracy versus the Signal to Noise ratio (SNR), defined as $\textrm{SNR}:=10\textrm{log}_{10}\left (\frac{\sigma^2_{\mathcal{T}}}{\sigma^2_{\epsilon}} \right)$, where $\sigma^2_{\mathcal{T}}$ is the variance of the data used for training our model. The proposed AA-GCN architecture is  compared with the Selection EDS architecture from \cite{gama2018convolutional}, and the graph coarsening strategy from \cite{defferrard2016convolutional}. As we can notice from Fig. 3, the proposed AA-GCN outperforms its competitors, illustrating its good capability to mitigate the effect of an additive noise on training data.



\subsection{Insights and Observations}
Lorem ipsum dolor sit amet, consectetur adipiscing elit, sed do eiusmod tempor incididunt ut labore et dolore magna aliqua. Ut enim ad minim veniam, quis nostrud exercitation ullamco laboris nisi ut aliquip ex ea commodo consequat. Duis aute irure dolor in reprehenderit in voluptate velit esse cillum dolore eu fugiat nulla pariatur. Excepteur sint occaecat cupidatat non proident, sunt in culpa qui officia deserunt mollit anim id est laborum.

==> Tables/acc_learn_to_rewire_authorship.tex <==
\begin{table}[t]
\centering
\caption{Best accuracy for authorship attribution.}
\resizebox{.45\linewidth}{!}{
\begin{tabular}{l|c}
\multicolumn{1}{l|}{Architecture} & \multicolumn{1}{c}{Accuracy} \\ \hline
Selection Degree               &65.7\,($\pm$9.12)\%                 \\
Selection EDS                  &75.4\,($\pm$2.7)\%                 \\
Selection SP                   &67.8\,($\pm$11.5)\%                 \\
Aggregation Degree             &70.5\,($\pm$2.0)\%                 \\
Aggregation EDS                &71.0\,($\pm$2.8)\%                 \\
Aggregation SP                 &73.5\,($\pm$3.4)\%                 \\
Multinode Degree               &82.8\,($\pm$3.3)\%                 \\
Multinode EDS                  &80.5\,($\pm$2.6)\%                 \\
Multinode SP                   &82.2\,($\pm$2.4)\%                 \\
Graph Coarsening               &87.9\,($\pm$2.2)\%                 \\
Autoencoder Aided              &\textbf{90.3\,($\pm$2.7)\%}              
\end{tabular}%
}
\end{table}\label{tab:authorship}
